Real-time Remote Tracking and Autonomous Planning for Whale Rendezvous using Robots

We introduce a system for real-time sperm whale rendezvous at sea using an autonomous uncrewed aerial vehicle. Our system employs model-based reinforcement learning that combines in situ sensor data with an empirical whale dive model to guide navigation decisions. Key challenges include (i) real-time acoustic tracking in the presence of multiple whales, (ii) distributed communication and decision-making for robot deployments, and (iii) on-board signal processing and long-range detection from fish-trackers. We evaluate our system by conducting rendezvous with sperm whales at sea in Dominica, performing hardware experiments on land, and running simulations using whale trajectories interpolated from marine biologists' surface observations.

==> text/algorithm.tex <==
\begin{algorithm}
\caption{\textcolor{blue}{Localization module Complete}}
\begin{algorithmic}[1]
\REQUIRE $k\gets$ maximum number of whales $\mathcal{A}\gets$ acoustic AOA, $\mathcal{V}\gets$ VHF AOA
\ENSURE Belief location and surface status of tracked whales

\STATE
$w^i \gets $ sample locations which are $\delta^i$ distance from the boat with angles $ \theta_{boat}+\alpha^i, \theta_{boat}-\alpha^i$, where $\alpha^i$ is the initial angle, $\theta_{boat}$ is the boat's heading

\FOR{every 10 seconds}
\STATE  $n\in \argmin_{m=[1,\cdots,k]} BIC(GMM(\mathcal{A}, m))$
 and 
$\{ \mu^j_\alpha, \sigma^j_\alpha \}^{n}_{j=1} \gets$  $GMM(\mathcal{A}, n)$
\STATE $I\gets Assign\_acoustic\_AOA\_to\_whale\_id(\mathcal{A})$
\STATE $J\gets Assign\_VHF\_AOA\_to\_whale\_id(\mathcal{V})$
\IF{whale $i\notin I$ is silent for $\delta_{silent}$ time steps or VHF is available for whale $i\in J$}
\STATE $surface\_status^i\gets$ surface
\ENDIF
\FOR {$i$ in $I$}
\STATE
$w^i\gets PF\_Update(\mu^i_\alpha, \sigma^i_\alpha)$
\IF {particles are degenerated}
\STATE 
$w^i \gets $ sample locations which are $\delta^i\sim \mathcal{U}(0,1000)$ distance from the boat with angles $ \theta_{boat}+\alpha^i$ and $\theta_{boat}-\alpha^i$
% $w^i \gets \{ PF(\theta_{boat}+\alpha^i, \delta^i), PF(\theta_{boat}-\alpha^i, \delta) \}, \alpha^i \sim \mathcal{N}(\mu^i_\alpha, (\sigma^i_\alpha)^2), \delta^i\sim \mathcal{U}(0,1000)$
\ENDIF
%     \IF{$A[i] > max$}
%         \STATE $max \leftarrow A[i]$
%     \ENDIF
\ENDFOR
\STATE $\iota \in \argmin dist(boat\_location, whale\_belief)$
\IF{time \% $\delta_t$ == 0, where $\delta_t$ is the boat maneuver decision interval duration}
\IF{Amplitude$(\iota)<$ threshold} 
\STATE Boat turns directly to  whale $\iota$
\ELSE 
\STATE Boat turn angle $\delta_\theta \in argmin_{\theta\in [-90,0,90]}{dist(new\_boat\_location(\theta, \delta_t), w^\iota)} $
% \STATE Take a turn with angle $\delta_\theta$ 
\ENDIF

\ENDIF
\STATE Take a 180 degree turn if $\alpha^\iota>90$ after 1 minute of each boat maneuver decision

\ENDFOR
\RETURN belief locations and surfacing status for whales
\label{Algo:localization}
\end{algorithmic}
\end{algorithm}


==> text/problem.tex <==
\section{Problem} \label{problem}
Achieving in situ rendezvous requires real-time data collection, processing, and decision-making to better predict and respond to events based on in situ sensing. We formulate our problems as follows:

\subsection{In Situ Localization}
The linear hydrophone array introduces \textit{directional ambiguity} in acoustic AOA sensing~--- signals originating from the left and right of the array are indistinguishable. In effect, this restricts the range of possible acoustic AOA estimates from $[0, 2\pi)$ to $[0, \pi]$ and \sg{can} lead to quickly compounding localization errors. 

In addition, the acoustic hydrophone \sg{senses acoustic signals from multiple sources simultaneously, including vocalizing whales as well as background noise.} In the presence of two or more groups of whales in spatially disparate locations, we must identify acoustic AOA estimates originating from each group and localize each group individually. We refer to this localization subproblem as \textit{group separation}. We note that this is a relaxation to the source separation problem studied in \cite{Diamant2025}, which aims to match acoustic signals to individual whales based on their vocal characteristics rather than spatially proximate groups.

When a whale is tagged, VHF-based sensing offers a complementary approach for surface localization since VHF AOA is an available sensing modality at the surface, unlike acoustic AOA. To achieve this, we must develop long-range real-time sensing capabilities and compute VHF AOA for off-the-shelf VHF fish-trackers. \sg{NOTE: I removed the sentence about directionality for VHF - VHF can also suffer from directionality issues if your antenna array is linear - let's not go here since its too much detail.}

\subsection{Decision-Making for UAV Navigation}
We formulate the real-time rendezvous problem as the partially observable sequential decision-making problem, where a belief $b =(b^1, \cdots, b^M)$ is represented as a collection of $M$ belief particles. 
Each belief particle $b^m$ consists of (i) the UAV's location and remaining flight time, (ii) the whale's estimated location, and (iii) a possible whale surface schedule sampled from the Gaussian distributions of underwater and surface durations $\mathcal{N}(\mu_{underwater}, \sigma_{underwater})$ and $\mathcal{N}(\mu_{surface}, \sigma_{surface})$, respectively (according to \cite{Gero2014BehaviorAS}). 
The flying status $f \in \{\texttt{grounded}, \texttt{in-flight}\}$, determines the available actions: $\{\texttt{takeoff},\texttt{wait}\}$ when \texttt{grounded} or $\{\texttt{go home},$ $\texttt{follow belief}\}$ when \texttt{\{in-flight}\}, respectively.


We want to find the UAV's navigation policy $\tilde{\mu}(b,f)$ over all possible actions $U_f$ at the belief state $b$ that minimizes the expected total time of rendezvous with the whale. \sg{SG NOTE: the description of ``minimizing expected total time of rendezvous with the whale'' is not clear. What does this mean? It sounds like it could mean minimize the time that the drone is with the whale...  Do you mean minimize the time from takeoff to successful visual rendezvous with the whale? Is this one rendezvous or several sequential rendezvouses? Please make this more specific}

\begin{equation}
\tilde{\mu}(b,f) \triangleq \argmin_{u \in U_f}\Big\{
     \mathbb{E}_m[ g(b^m,u) + J(F(b^m,u))] \Big\} 
\label{eq:drone_rollout}
\end{equation}
where $g(b^m, u)$ is the minimum of either the time taken to finish action $u$ for belief particle $b^m$, or a pre-defined maximum number of time steps. The transition function $F(b^m,u)$ gives the next belief particle given the current belief particle and action. The cost function $J(\cdot)$ is the time to complete rendezvous with considerations to the remaining fight time of the UAV under maximum speed and distance between the whale particle over the planning horizon. \sg{SG NOTE: It is not clear from this description how to compute $J$ and how ``considerations to the remaining flight time'' is taken into account. Importantly, this needs to be described in enough details that others can implement it. Can you expound on these terms and how to compute them? Can you provide explicit forms for the functions $g$, $J$? What is $m$? Is this the number of particles? Is this a random variable?  What is meant by expectation over $m$? Please explain.} 
% We estimate $J(.)$ by greedily navigating towards the whale locations until battery depletion if the UAV is in the in-flight, other-wise we wait t.

\subsection{Real-time Deployment}
In situ operations require integrating multiple sensing modalities, real-time UAV deployment, and beyond-line-of-sight autonomous flight. To meet these demands, we need to design a system deployable on a catamaran platform, enabling distributed communication between the decision-making module, sensors, and UAV.
